Better Generalization with Semantic IDs: A Case Study in Ranking for Recommendations

Randomly-hashed item ids are used ubiquitously in recommendation models. However, the learned representations from random hashing prevents generalization across similar items, causing problems of learning unseen and long-tail items, especially when item corpus is large, power-law distributed, and evolving dynamically. In this paper, we propose using content-derived features as a replacement for random ids. We show that simply replacing ID features with content-based embeddings can cause a drop in quality due to reduced memorization capability. To strike a good balance of memorization and generalization, we propose to use Semantic IDs -- a compact discrete item representation learned from frozen content embeddings using RQ-VAE that captures the hierarchy of concepts in items -- as a replacement for random item ids. Similar to content embeddings, the compactness of Semantic IDs poses a problem of easy adaption in recommendation models. We propose novel methods for adapting Semantic IDs in industry-scale ranking models, through hashing sub-pieces of of the Semantic-ID sequences. In particular, we find that the SentencePiece model that is commonly used in LLM tokenization outperforms manually crafted pieces such as N-grams. To the end, we evaluate our approaches in a real-world ranking model for YouTube recommendations. Our experiments demonstrate that Semantic IDs can replace the direct use of video IDs by improving the generalization ability on new and long-tail item slices without sacrificing overall model quality.

==> 3_background.tex <==
%This section presents key aspects of the video ranking system at YouTube. These factors provide context and define the constraints and requirements we must consider.

%\textsl{Ranker Model:} Our production ranking model is a multitask model for video recommendation~\cite{Tang_2023, mtlranking}, which recommends the next video to watch, given a video a user is watching. The hidden layers in the model are shared across the multiple training tasks. Prior to our work on Semantic IDs, video ID features were the most essential features of the model. The current video and the video to be ranked were represented as video IDs. Furthermore, a user was also represented as a sequence of video IDs they interacted with - a critical feature to make the recommendation more personalized.

%\textsl{Content Embeddings:} In our work, we use a video encoder developed in-house to generate content embeddings for each YouTube video. The video encoder is a transformer model that uses VideoBERT ~\cite{videoBert} as the backbone architecture, takes audio and visual features as inputs, and outputs $2048$-dimensional embeddings that capture the topicality of the video. This model was trained using techniques described in ~\cite{Lee_2020_CVPR}.

% These embeddings capture the topicality of the video and the video encoder 
% There exists systems in place to annotate YouTube videos with multimodal content embeddings that capture the topicality of the video. The video encoder incorporates visual and audio information about the video, 
% Videos are annotated by video embeddings
% We use a $256$ dimensional frozen content embedding from a video encoder that incorporates visual and audio information about the video as the input to the RQ-VAE model. The video encoder uses video BERT ~\cite{videoBert} as the backbone architecture and was trained using techniques described in ~\cite{Lee_2020_CVPR}.
%As discussed in Section~\ref{sec:1_introduction}, we use the hashing trick~\cite{weinberger2009feature} on the video IDs to train the  embeddings.

%Of the many sparse and dense features that the model takes as input, video IDs based features are the most important. Video IDs are used to represent both current and   

%While some systems represent users by user IDs~\cite{}, we instead rely on using the watch history (list of video IDs user interacted with in the past) to represent the users, to generate personalized recommendations. 
% \textsl{Sequential Training:} We train the ranking model sequentially, i.e., the training is done using logged data chronologically, and the training continues as new data come in. Since the underlying video corpus and users constantly evolve, the model must generalize well under a data-distribution shift. Hence, in this paper, we evaluate our methods on the data that the trained model has not yet seen. This allows us to understand the performance under the data-distribution shift of the video corpus.

%\textsl{Resource Constraints:}
%Due to resource constraints and latency budgets dictated by real-time inference, we cannot increase resource usage significantly.
%For example, a possible approach to avoid video IDs is directly using content embeddings as input to the model. However, this approach is not viable due to high resource costs. For instance, storing 100s of 2048-dimension floats to represent users' watch history per training example for industrial applications with billions of examples blows up storage usage. Loading and processing such large inputs also significantly slows down training and increases latency at inference. Furthermore, if we use content embeddings to replace video IDs, we lose the model capacity associated with the video embedding parameters, leading to model quality degradation. In theory, we can increase the hidden layer capacity to compensate. However, this increases computational costs in practice since model capacity in dense layers is much more compute-heavy than embedding parameters. Due to resource constraints and latency budgets dictated by real-time inference, adopting this approach is not feasible.
